Practitioner-Centric Approach for Early Incident Detection Using Crowdsourced Data for Emergency Services

Emergency response is highly dependent on the time of incident reporting. Unfortunately, the traditional approach to receiving incident reports (e.g., calling 911 in the USA) has time delays. Crowdsourcing platforms such as Waze provide an opportunity for early identification of incidents. However, detecting incidents from crowdsourced data streams is difficult due to the challenges of noise and uncertainty associated with such data. Further, simply optimizing over detection accuracy can compromise spatial-temporal localization of the inference, thereby making such approaches infeasible for real-world deployment. This paper presents a novel problem formulation and solution approach for practitioner-centered incident detection using crowdsourced data by using emergency response management as a case-study. The proposed approach CROME (Crowdsourced Multi-objective Event Detection) quantifies the relationship between the performance metrics of incident classification (e.g., F1 score) and the requirements of model practitioners (e.g., 1 km. radius for incident detection). First, we show how crowdsourced reports, ground-truth historical data, and other relevant determinants such as traffic and weather can be used together in a Convolutional Neural Network (CNN) architecture for early detection of emergency incidents. Then, we use a Pareto optimization-based approach to optimize the output of the CNN in tandem with practitioner-centric parameters to balance detection accuracy and spatial-temporal localization. Finally, we demonstrate the applicability of this approach using crowdsourced data from Waze and traffic accident reports from Nashville, TN, USA. Our experiments demonstrate that the proposed approach outperforms existing approaches in incident detection while simultaneously optimizing the needs for real-world deployment and usability.

==> sections/data.tex <==
\section{Data}
\label{sec:data_platforms}

\textcolor{red}{smv:if we run out of space, we  can summarize sections 4.1 to 4.4 in just one table and a paragraph}

\textcolor{red}{smv: approach 1: Long version}

\subsection{Waze Data Set}
\label{sec:waze_data}
% Describe Waze data -- copied from Previous paper

Waze is a crowdsourcing platforms which allows us to collect information about incidents using the observations reported by the users ~\cite{waze_driving_2020}. The Waze data was available from Sep/01/2019 to Dec/31/2019. The most relevant attributes used in this paper are summarized in the following. 

\begin{itemize}
    \item \textbf{uuid}:  A unique ID for each report provided by Waze.
    \item \textbf{confidence}: Based on other users' reactions to a report ("Thumbs up" or "Not There"), each alert receives a score between [0-10], where lower value shows more negative feedback. %created by the reporting user.
    \item \textbf{location}: Longitude and latitude of the report origin using WGS 1984 spatial reference.
    \item \textbf{pubMillis}: Each alert has a timestamp, which is in milliseconds since epoch. 
    \item \textbf{reliability}: Each alert receive a reliability score between [1-10] based on  based on \textit{reportRating} scores of the reporters and other user’s reactions \textit{confidence}. The higher the  reliability score, the more reliable the report.  
    
    %\textcolor{red}{smv: I checked on internet and it seems reliability just depends on reporters reportRating while in your previous paper you mentioned that it depends on both  reportRating and confidence. Please double check.  -- Yasas: pls check comment}   
    
    \item \textbf{reportRating}: Waze reporters obtain experience levels  between [1-6] based on their contributions. The lower value indicates the less experienced and reliable the reporter is. 
    \item \textbf{type}: Type of traffic alert; traffic alerts with type `ACCIDENT' are of interest of this study. 
\end{itemize} 


\subsection{Incident Data Set and Labels} \textcolor{red}{smv: what does Lables mean here?}
\label{sec:incident_data}
Through collaboration with Nashville Fire Department (NFD) \cite{NFD}, a data set including all the incidents responded by NFD between years 2017 and 2021 is available. The incidents in this data set are considered as the ground truth or the actual accidents, which we aimed to predict. In this study, just Traffic/Transportation incidents are of interest. Also, each incident is allocated to its closest  closest roadway segment as long as the distance is less than 25 m. Roadway segment are based on INRIX traffic data set. The most relevant attributes used in this paper are summarized in the following. \textcolor{red}{smv: please let me know if there is a feature that you used but it is not here. Also, if there is a feature that you didnt use but it is here, please mark it and we can delete it later}. 

\begin{itemize}
    \item \textbf{ID}: A unique ID for each incident provided by NFD.
    \item \textbf{Coordinates}: Longitude and latitude of the location of incident using WGS 1984 spatial reference.
    \item \textbf{emdCardNumber}:  It is dispatch determinants (codes) utilized in the Priority Dispatching system. In other, it defines the type of the mission. Protocol 29 includes Traffic/Transportation incidents.
    \item \textbf{time}: Timestamp for time the incident was reported to NFD.
    \item \textbf{XDSegID}: The ID of closest roadway segment.
    \item \textbf{Dist to Seg}: Distance to closest roadway segment in meter.
\end{itemize} 


\subsection{Traffic Data Set}
Traffic data is one of the most effective features in accident prediction~\cite{mukhopadhyay2020review}. For this study and for the time range of interest, the 5-minute temporal resolution traffic data of roadway segments in Nashville area is collected from INRIX \cite{inrix}. Furthermore, each roadway segment is mapped to the closest weather station. The collected features are outlined below.

\begin{itemize}
    \item \textbf{xd id}: A unique ID for each roadway segment provided by INRIX.
    \item \textbf{measurement tstamp}: Representing the start of the reading's time window.
    \item \textbf{average speed}:  Representing the historical average speed each segment for each hour of day and for each day of the week.
    \item \textbf{speed}: The current estimated harmonic mean speed for the roadway segment in miles per hour.
    \item \textbf{reference speed}: The calculated \textit{free flow speed} for the roadway segment in miles per hour.
    \item \textbf{confidence score}: A confidence score regarding the accuracy of the traffic data.
    \item \textbf{cvalue}: Indicates the probability that the current reading represents the actual roadway conditions.
    \item \textbf{congestion}: It is the ratio of the difference between free flow speed and the current speed to free flow speed.
    \item \textbf{Station ID}: The ID of the closest weather station to this segment. 
\end{itemize} 

\textcolor{red}{Yasas is working on getting the setup for integrating -- taking some time. Yasas will update once done.}

\subsection{Weather Data Set}
The other important spatial temporal data set is the Weather data set, which is  collected hourly from weatherbit \cite{weatherbit}. In our model, for each segment, we use the weather data of the closest weather station.

\begin{itemize}
    \item \textbf{Visibility}:  A measure of the distance at which an object or light can be clearly discerned. The unit is km. 
    \item \textbf{Wind Speed }: Speed of wind in meter per second
    \item \textbf{Precipitation}: Amount of precipitation in mm. 
    \item \textbf{Temperature}: It is the reported temperature in Celsius.
    \item \textbf{Coordinates}: Longitude and latitude of the location of station using WGS 1984 spatial reference.
    \item \textbf{Station ID}: A unique ID for each station provided by weatherbbit.
    
\end{itemize}





















==> sections/related_work.tex <==
\section{Background and Related Work}
\label{sec:related}

\vspace{-0.05in}

%\textcolor{red}{This section was copied from our previous paper. Need to describe -- (1) Incident detection modeling (all data sources) (2) Crowdsourcing for incident detection (3) Optimal policy selection for user-centered system design}

% \subsection{Crowdsourced Data in Transportation Analytics}
%
% - discuss different domain for analytics (transportation, surveillance, ..) \\ 
%Crowdsourced data (such as Twitter, Instagram, Waze, and Foursquare) represents another source of data that has been used for a variety of analyses such as emergency disaster response \cite{purohit2018structured}, urban activity detection \cite{niu2020crowdsourced}, disease transmission \cite{chunara2013we}, and traffic management \cite{amin2018evaluating}. Since the focus of this paper is on road incidents, we review previous related work on the use of crowdsourced data for it. % 
%Transportation systems are the critical infrastructure of the modern cities. Therefore, significant research has been conducted to perform analytics on the transportation systems and traffic conditions using various sources of available data, including crowdsourced data. Hence, we provide a brief literature overview on the use of crowdsourced data for analyzing transportation systems. 
Recently, there has been a growing interest in leveraging user-generated, crowdsourced data for various public sector domains such as emergency management and transportation. % specifically traffic incident prediction. 
Crowdsourced data (such as Twitter, Instagram, Waze, and Foursquare) represents another source of data that has been used for a variety of analyses such as emergency disaster response\cite{senarath2020emergency},  %\cite{purohit2018structured},
% urban activity detection \cite{niu2020crowdsourced}, 
% disease transmission \cite{chunara2013we}, 
and traffic management \cite{amin2018evaluating}. 
% Silva et al \cite{silva2013traffic} studied the breadth and spatial coverage capabilities of the Waze report information to understand the traffic conditions, and also their limitations. They  concluded that the frequency of the Waze alerts is consistent with the users' routines and traffic patterns.
% 
% Sanchez et al. \cite{sanchez2019dynamic} investigated the impacts of dynamic traffic lighting by analyzing the traffic jam and traffic incident reports from Waze. The authors concluded that  dynamic traffic lighting can reduce traffic congestion and improve traffic speed but has no impact on the occurrence of traffic accidents.
%
%Santos et al. \cite{dos2017analyzing} also performed a comparative study between the official accident (BHTrans) and Waze datasets in the city of Belo Horizonte, Brazil, and found that there was a 7\% match in the accidents reported by both the datasets. When compared to Waze reports, the BHTrans data was spread more uniformly across the day. Most of the accidents reported by Waze but not by BHTrans were classified as having lower severity. Accidents reported only by BHTrans were concentrated on the central region of Belo Horizonte, while the ones reported by Waze were mostly on highway segments. 
% 
% Since we use traffic accidents as a use-case in this paper, we focus on prior work from the same domain.
Lenkei~\cite{lenkei2018crowdsourced} performed a comparative study of the accidents reported through Waze and the official traffic database in Sweden (Trafikverket), and concluded that there was a 43\% overlap in the accident data between Waze and Trafikverket. He also observed that 27.5\% of the incidents in Trafikverket were detected earlier by Waze.
% Eriksson \cite{eriksson2019towards} and Santos et al. \cite{dos2017analyzing} integrated accident data from the official accident database and Waze to create a comprehensive accident database after removing the data that were common in both the datasets through spatio-temporal proximity analysis. 
%
%% The author provided two reasons for the increased number of Waze alerts. First, some of the Waze alerts can either be self-resolving, false alarms, or of low impact. And, second, the Waze data stream can include multiple alerts referring to the same accident. 
%
%%The author built a binomial logistic regression model using a set of independent variables (type of alert, the type of the road where the incident happened, the part of the day when the incident happened, the rank of the reporter, the number of related alerts, the number of related jams and the number of confirmations that the alert has received) to determine if a Waze alert refers to an incident that should be handled by incident management authorities. 
% 
% Furthermore, Amin-Naseri et al.~\cite{amin2018evaluating} concluded that Waze reports can detect incidents earlier than probe-based methods with reasonable geographic accuracy. 
% Flynn et al.~\cite{flynn2018estimating} investigated the ability of Waze data to serve as a reliable indicator of police-reportable crashes through machine learning approaches. 
%[full] In particular, the authors considered a Random Forest (RF) model to predict the number of police-reportable crashes using weather, Waze reports (median report reliability, number of records, type of Waze event, road classification), time (hour of day and day of week), and urban area classification. 
Recently, Senarath et al. \cite{senarath2020emergency} described a Bayesian information fusion approach to fuse multiple crowdsourced Waze reports for incident detection. Moreover, they demonstrated early incident detection using Waze reports when compared against official incident records. 
%[full] Zhang et al.~\cite{zhang2021secondary} demonstrated the applicability of Waze incidence reports to identify secondary crashes (crashes due to non-recurrent congestion originating from primary crashes) that could not be identified from currently-used methods. 

% Moreover, Xi et al. \cite{li2020rethinking} demonstrated the significance of integrating traditional police crash reports with Waze incident reports to identify high risk road segments for data-driven highway safety analysis and decision-making. Their real-world study concluded that Waze and police reports are spatially correlated and that the Waze reports have a broader coverage with 60.24\% of sites receiving more Waze reports than the police reports. Through integration of Waze and police reports, their study identified 14 miles of high risk road segments when compared to 8 miles identified using only the police reports.


% explore the predictability of unconventional, \textit{noisy} Waze reports to detect emergency incidents, and especially, the need for a generic, principled approach for spatio-temporal information fusion of the \textit{redundant} and \textit{noisy} crowdsourced reports to detect emergency incidents.  

% The authors found that models could identify the number of actual police-reported crashes with high accuracy. Therefore, this method could be applied to incoming Waze data to estimate real-time spatio-temporal patterns in police-reportable crashes. Fire et al \cite{fire2012data} analyzed Waze reports in Israel, and discussed ways to improve the police coverage and resource allocation in regions with large number of accidents by comparing accident reports and reports of police sightings. So far, we discussed the applications of Waze data for traffic incident detection and traffic congestion. Below, we review the application of other types of crowdsourced data in traffic management.


% \subsection{Crowdsourced Data in Emergency Event Detection} 
% %
% A variety of crowdsourcing platforms have been investigated to detect real-world events in the past, which inspire our methodology for incident detection. Riberio et al \cite{ribeiro2014studying} concluded that the number of ``check-ins'' from FourSquare/Instagram and traffic condition data from Bing Maps are well correlated, and such crowdsourced data can be used to predict traffic congestion events. 
% % 
% Sakaki et al. \cite{sakaki2010earthquake} developed a combination of text classification and probabilistic Kalman filtering approaches for spatio-temporal localization and identification of earthquake events using Twitter data. 
% % 
% Zhou and Chen \cite{zhou2014event} developed a location-time constrained topic model to capture the interplay between content, time, and location of social media (Twitter) posts for detecting events. Using this model, posts are represented by probability distribution over a set of pre-defined topics, and the similar posts, measured by the distance between their associated probability distributions,
% are integrated for event detection. 
% % 
% Similarly, Cheng and Wicks \cite{cheng2014event} developed Twitter-based event detection technique using space-time scan statistics, which considered spatio-temporal clustering of tweets to identify new abnormal tweet clusters to identify an event of interest. Similar clustering-based approach was also developed by Hasan et al. \cite{hasan2016twitternews} for event detection.

%Based on the above review,
\textbf{Gaps:} We note that the existing approaches that use crowdsourced data for emergency incident detection lack: 
\begin{enumerate*}
    \item a principled approach for information fusion of redundant and noisy data to detect incidents that could be extended to various crowdsourcing platforms because the existing approaches consider only simple aggregation methods (count/average) of surface-level features without considering impacts of uncertainty associated with report integration; 
    \item a systematic investigation of the effect of hyperparameters (e.g. quality of discretization of a continuous region of interest to finite and discrete regions) on the quality and accuracy of the event detection models developed from crowdsourced data; 
    \item a flexible incident detection framework that accommodates practitioner preferences regarding incident detection accuracy and spatial-temporal localization.
\end{enumerate*}
We address these issues in our proposed approach.







==> tables/feature_table.tex <==

\begin{table*}[]
\centering
\caption{Data Description (the name of the partner city is suppressed for blind review)}
\resizebox{0.9\textwidth}{!}{%
%\begin{tabular}{|l|l|l|l|l|l|}
\begin{tabular}{|l|l|l|l|l|p{0.5\linewidth}|}
\hline
\multicolumn{1}{|l|}{Dataset} & \multicolumn{1}{l|}{Frequency} & Feature & Source & Type & Explanation \\ \hline
\multirow{5}{2cm}{Crowsourced Reported Incident} & \multirow{5}{*}{Continuous} & ID & Waze & Spatio-temporal & A unique ID for each report provided by Waze. \\ \cline{3-6} 
  &  & Coordinates & Waze & Spatio-temporal & Longitude and latitude of the report origin using WGS 1984   spatial reference. \\ \cline{3-6} 
  &  & Time & Waze & Spatio-temporal & Each alert has a timestamp, which is in milliseconds since   epoch. \\ \cline{3-6} 
  &  & Reliability & Waze & Spatio-temporal & Each alert receive a reliability score between {[}1-10{]} based   on  \textit{reportRating}   scores of the reporters and other user’s reactions \textit{confidence}. \\ \cline{3-6} 
  &  & Type & Waze & Spatio-temporal & Type of traffic alert; traffic alerts with type `ACCIDENT' are   of interest of this study. \\ \hline
\multicolumn{1}{|l|}{\multirow{6}{*}{Actual Incident}} & \multicolumn{1}{l|}{\multirow{6}{*}{Continuous}} & ID & Partner City & Spatio-temporal & A unique ID for each incident provided by Partner City. \\ \cline{3-6} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & Coordinates & Partner City & Spatio-temporal & Longitude and latitude of the location of incident using WGS   1984 spatial reference. \\ \cline{3-6} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & Type & Partner City & Spatio-temporal & Dispatch determinants or the type of the incident. We focus on Traffic/Transportation incidents. \\ \cline{3-6} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & Time & Partner City & Spatio-temporal & Timestamp for time the incident was reported to Partner City. \\ \cline{3-6} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & XDSegID & Derived & Spatio-temporal & ID of closest roadway segment. \\ \cline{3-6} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & Dist to Seg & Derived & Spatio-temporal & Distance to closest roadway segment in meter. \\ \hline
\multirow{5}{*}{Traffic} & \multirow{5}{*}{5 minutes} & XDSegID & INRIX & Spatio-temporal & A unique ID for each roadway segment provided by INRIX. \\ \cline{3-6} 
  &  & Time & INRIX & Spatio-temporal & Representing the start of the reading's time window \\ \cline{3-6} 
  &  & Speed & INRIX & Spatio-temporal & The current estimated harmonic mean speed for the roadway   segment in miles per hour. \\ \cline{3-6} 
  &  & Reference Speed & INRIX & Spatial & The calculated \textit{free flow speed} for the roadway segment   in miles per hour. \\ \cline{3-6} 
  &  & Congestion & Derived & Spatio-temporal & Congestion is the ratio of the difference between free flow   speed and the current speed to free flow speed. \\ \hline
\multirow{3}{*}{Weather} & \multirow{3}{*}{1 hour} & Station ID & Weatherbit & Spatial & A unique ID for each station provided by weatherbbit. \\ \cline{3-6} 
  &  & Precipitation & Weatherbit & Spatio-temporal & Amount of precipitation in mm. \\ \cline{3-6} 
  &  & Coordinates & Weatherbit & Spatio-temporal & Longitude and latitude of the location of station using WGS 1984   spatial reference. We use this to find the closest station to each grid   cell. \\ \hline
\end{tabular}
}
\label{table:datasets}
\end{table*}

==> tables/feature_table_min.tex <==

\begin{table}[]
\centering
\caption{Data Description}
\resizebox{0.5\textwidth}{!}{%
%\begin{tabular}{|l|l|l|l|l|l|}
\begin{tabular}{|l|p{1.5cm}|p{0.8\linewidth}|}
\hline
\textbf{Dataset} & \textbf{Feature} & Explanation \\ \hline
\multicolumn{1}{|c|}{
\multirow{5}{1.5cm}{Crowsourced Reported Incident}
} & ID & A unique ID for each report provided by Waze. \\ \cline{2-3} 
\multicolumn{1}{|c|}{} & Coordinates & Longitude and latitude of the report origin using WGS 1984   spatial reference. \\ \cline{2-3} 
\multicolumn{1}{|c|}{} & Time & Each alert has a timestamp, which is in milliseconds since   epoch. \\ \cline{2-3} 
\multicolumn{1}{|c|}{} & Reliability & Each alert receive a reliability score between {[}1-10{]} based   on  \textit{reportRating}   scores of the reporters and other user’s reactions \textit{confidence}. \\ \cline{2-3} 
\multicolumn{1}{|c|}{} & Type & Type of traffic alert; traffic alerts with type `ACCIDENT' are   of interest of this study. \\ \hline
\multirow{6}{1.5cm}{Actual Incident} & ID & A unique ID for each incident provided by Partner City. \\ \cline{2-3} 
 & Coordinates & Longitude and latitude of the location of incident using WGS   1984 spatial reference. \\ \cline{2-3} 
 & Type & Dispatch determinants or the type of the incident. We focus on Traffic/Transportation incidents. \\ \cline{2-3} 
 & Time & Timestamp for time the incident was reported to Partner City. \\ \cline{2-3} 
 & XDSegID & ID of closest roadway segment. \\ \cline{2-3} 
 & Dist to Seg & Distance to closest roadway segment in meter. \\ \hline
\multirow{5}{*}{Traffic} & XDSegID & A unique ID for each roadway segment provided by INRIX. \\ \cline{2-3} 
 & Time & Representing the start of the reading's time window \\ \cline{2-3} 
 & Speed & The current estimated harmonic mean speed for the roadway   segment in miles per hour. \\ \cline{2-3} 
 & Reference Speed & The calculated \textit{free flow speed} for the roadway segment   in miles per hour. \\ \cline{2-3} 
 & Congestion & Congestion is the ratio of the difference between free flow   speed and the current speed to free flow speed. \\ \hline
\multirow{3}{*}{Weather} & Station ID & A unique ID for each station provided by weatherbit. \\ \cline{2-3} 
 & Precipitation & Amount of precipitation in mm. \\ \cline{2-3} 
 & Coordinates & Longitude and latitude of the location of station using WGS 1984   spatial reference. We use this to find the closest station to each grid   cell. \\ \hline
\end{tabular}
}
\label{table:datasets}
\vspace{-0.2in}
\end{table}

==> tables/hyperparam_table.tex <==
\begin{table}[]
\centering
\caption{Hyperparameters selected for CNN model based on a cross-validation.}
\label{tab:model-params}
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{|l|l|r|}
\hline
\textbf{Layer} & \textbf{Parameter} & \multicolumn{1}{l|}{\textbf{Value}} \\ \hline
\multirow{2}{*}{Convolution} & \# of Filters & 256 \\ \cline{2-3} 
 & Kernel Size & (2, 2) \\ \hline
\multirow{2}{*}{Pooling} & Type & Max \\ \cline{2-3} 
 & Pool Size & (2, 2) \\ \hline
\multirow{2}{*}{Convolution} & \# of Filters & 256 \\ \cline{2-3} 
 & Kernel Size & (2, 2) \\ \hline
\multirow{2}{*}{Hidden (Dense)} & \# of Units & $2 \times N_{o}$ \\ \cline{2-3} 
 & Activation & ReLU \\ \hline
\multirow{2}{*}{Output (Dense)} & \# of Units & $N_{o}$ \\ \cline{2-3} 
 & Activation & Sigmoid \\ \hline
\end{tabular}%
}
\vspace{-0.2in}
\end{table}
